FAMOUS: High-Fidelity Monocular 3D Human Digitization Using View Synthesis

The advancement in deep implicit modeling and articulated models has significantly enhanced the process of digitizing human figures in 3D from just a single image. While state-of-the-art methods have greatly improved geometric precision, the challenge of accurately inferring texture remains, particularly in obscured areas such as the back of a person in frontal-view images. This limitation in texture prediction largely stems from the scarcity of large-scale and diverse 3D datasets, whereas their 2D counterparts are abundant and easily accessible. To address this issue, our paper proposes leveraging extensive 2D fashion datasets to enhance both texture and shape prediction in 3D human digitization. We incorporate 2D priors from the fashion dataset to learn the occluded back view, refined with our proposed domain alignment strategy. We then fuse this information with the input image to obtain a fully textured mesh of the given person. Through extensive experimentation on standard 3D human benchmarks, we demonstrate the superior performance of our approach in terms of both texture and geometry. Code and dataset is available at https://github.com/humansensinglab/FAMOUS.

==> sections/datasets.tex <==
\item $\bullet$  We mainly adapt the render people dataset which consists of 950 scans. We use 865 scans for training and 85 scans for testing. 

\item $\bullet$ \textcolor{red}{To verify the generality of FAMOUS we test on Deep Fashion dataset.} 

\item $\bullet$ All 3D scans are rendered using OpenGl scripts at every 10 degree yaw angle interval and obtain corresponding SMPLX fits and segmentation maps from PyMAFX. 

\item $\bullet$  For the 2D dataset we use Deep Fashion HD training images with original training pairs. 

\item $\bullet$ For the occupancy network and texture aggregation we only considered rendering with yaw angle [0, 180]. 

\color{teal}
\noindent \textbf{Datasets: } We employ RenderPeople \cite{renderpeople} dataset for the evaluation which consists of 950 3D scans \textcolor{red}{of how many subjects?}. We use 865 of those for training and the rest 85 scans for evaluation. These splits will be open-sourced with our codebase for reproducibility. The 2D renderings from these scans are generated at a $10\degree$ yaw interval. Moreover, the SMPLX fits and the corresponding segmentation maps are obtained with PyMAFX \cite{pymafx}. We resort to DeepFashion \cite{deep-fashion} as our 2D fashion dataset. The high-resolution pairs of the original training split from DeepFashion are used for the training following our vanilla hallucinator \cite{nted}.
\color{black}
